MedCutMix: A Data-Centric Approach to Improve Radiology Vision-Language Pre-training with Disease Awareness

Vision-Language Pre-training (VLP) is drawing increasing interest for its ability to minimize manual annotation requirements while enhancing semantic understanding in downstream tasks. However, its reliance on image-text datasets poses challenges due to privacy concerns and the high cost of obtaining paired annotations. Data augmentation emerges as a viable strategy to address this issue, yet existing methods often fall short of capturing the subtle and complex variations in medical data due to limited diversity. To this end, we propose MedCutMix, a novel multi-modal disease-centric data augmentation method. MedCutMix performs diagnostic sentence CutMix within medical reports and establishes the cross-attention between the diagnostic sentence and medical image to guide attentive manifold mix within the imaging modality. Our approach surpasses previous methods across four downstream radiology diagnosis datasets, highlighting its effectiveness in enhancing performance and generalizability in radiology VLP.

==> tables/main_results.tex <==
\begin{table}[t!]
\centering
\caption{Main results.}
\label{main_results}
\setlength\tabcolsep{4.0pt}
\renewcommand\arraystretch{1.5}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cc|cc|cc|cc|cc|c|c}
\toprule[1.5pt]
                  & \multicolumn{2}{c|}{CheXpert5} & \multicolumn{2}{c|}{CheXpert14} & \multicolumn{2}{c|}{PadChest} & \multicolumn{2}{c|}{NIH Chest Xray14} & \multicolumn{2}{c|}{RSNA} &          &         \\
                  & AUC            & F1            & AUC            & F1             & AUC           & F1            & AUC               & F1                & AUC         & F1          & Avg. AUC & Avg. F1 \\ \hline
MGCA              & 0.8452         & 0.4491        & 0.7122         & 0.3366         & 0.6855        & 0.0371        & 0.6057            & 0.1558            & 0.7206      & 0.5275      & 0.71384  & 0.30122 \\ \hline
MGCA w/ MedCutMix & 0.8535         & 0.4638        & 0.7137         & 0.342          & 0.689         & 0.0376        & 0.6202            & 0.1556            & 0.7278      & 0.5515      & 0.72084  & 0.3101  \\ \hline
GLoRIA            & 0.7203        & 0.2211         & 0.6324         & 0.2075         & 0.6131        & 0.0308       & 0.5809             & 0.1562            & 0.7509      & 0.6564      & 0.65952  & 0.2544         \\ \hline
GLoRIA w/ MedCutMix & 0.7207        & 0.1911        & 0.614          & 0.1561        & 0.6802        & 0.0433       & 0.5638            & 0.1513           & 0.7581      & 0.6228     & 0.66736  & 0.23292        \\ \bottomrule[1.5pt]
\end{tabular}
}
\end{table}
